BoMD: Bag of Multi-label Descriptors for Noisy Chest X-ray Classification

Deep learning methods have shown outstanding classification accuracy in medical imaging problems, which is largely attributed to the availability of large-scale datasets manually annotated with clean labels. However, given the high cost of such manual annotation, new medical imaging classification problems may need to rely on machine-generated noisy labels extracted from radiology reports. Indeed, many Chest X-ray (CXR) classifiers have already been modelled from datasets with noisy labels, but their training procedure is in general not robust to noisy-label samples, leading to sub-optimal models. Furthermore, CXR datasets are mostly multi-label, so current noisy-label learning methods designed for multi-class problems cannot be easily adapted. In this paper, we propose a new method designed for the noisy multi-label CXR learning, which detects and smoothly re-labels samples from the dataset, which is then used to train common multi-label classifiers. The proposed method optimises a bag of multi-label descriptors (BoMD) to promote their similarity with the semantic descriptors produced by BERT models from the multi-label image annotation. Our experiments on diverse noisy multi-label training sets and clean testing sets show that our model has state-of-the-art accuracy and robustness in many CXR multi-label classification benchmarks.

==> table_ablation.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{0.85\textwidth}{!}{  
    \begin{tabular}{c||c||cc||c||cc||c||cc||c||cc}
    \toprule
    \multirow{1}{*}{Experiments} & \multicolumn{6}{c||}{Mixup Coefficient}                   & \multicolumn{3}{c||}{Number of Descriptors} & \multicolumn{3}{c}{K-nearest neighbour}  \\ \midrule \midrule
    \multirow{1}{*}{Settings}    & $\lambda$    & OpenI             & PadChest & $\gamma$    & OpenI             & PadChest & $M$       & OpenI          & PadChest       & $K$       & OpenI       & PadChest      \\ \midrule
    \multirow{6}{*}{AUC}         
    &	0.2	&	88.39	&	85.52	&	0.05	&	89.14	&	86.05	&	1	&	88.34	&	86.02	&	5	&	89.20	&	86.15	\\
    &	0.4	&	88.56	&	85.93	&	0.15	&	87.87	&	86.17	&	3	&	\textbf{89.52}	&	\textbf{86.50}	&	10	&	\textbf{89.52}	&	\textbf{86.50}	\\
    &	0.6	&	\textbf{89.52}	&	\textbf{86.50}	&	0.25	&	\textbf{89.52}	&	\textbf{86.50}	&	5	&	88.92	&	86.39	&	20	&	88.23	&	85.79	\\
    &	0.8	&	88.37	&	86.29	&	0.35	&	88.40	&	86.48	&	7	&	89.03	&	86.43	&	50	&	87.59	&	85.49	\\
    &	1.0	&	88.31	&	86.21	&	0.45	&	88.46	&	86.46	&	9	&	88.45	&	86.29	&	100	&	87.36	&	85.48	\\
	\bottomrule													
    \end{tabular}
    }
    \caption{Ablation study of the hyper-parameters using mean AUC. Models are trained on NIH~\cite{nih} and tested on OpenI~\cite{openi} and PadChest~\cite{padchest}. Note that for each hyper-parameter, we fix the others to their best values (i.e., $\lambda=0.6$, $\gamma=0.25$, $M=3$ and $K=10$).}
    \label{tab:ablation}
    \vspace{-5pt}
\end{table*}
